JEN-1: Text-Guided Universal Music Generation with Omnidirectional Diffusion Models

Music generation has attracted growing interest with the advancement of deep generative models. However, generating music conditioned on textual descriptions, known as text-to-music, remains challenging due to the complexity of musical structures and high sampling rate requirements. Despite the task's significance, prevailing generative models exhibit limitations in music quality, computational efficiency, and generalization. This paper introduces JEN-1, a universal high-fidelity model for text-to-music generation. JEN-1 is a diffusion model incorporating both autoregressive and non-autoregressive training. Through in-context learning, JEN-1 performs various generation tasks including text-guided music generation, music inpainting, and continuation. Evaluations demonstrate JEN-1's superior performance over state-of-the-art methods in text-music alignment and music quality while maintaining computational efficiency. Our demos are available at https://jenmusic.ai/audio-demos

==> section/0-conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%complex version%%%%%%%%%%%
In this work, we have proposed JEN-1, a powerful and efficient text-to-music generation framework that outperforms existing methods in both efficiency and quality of generated samples. By directly modeling waveforms instead of mel-spectrograms, combining auto-regressive and non-auto-regressive training, and utilizing multi-task training objectives, JEN-1 is able to generate high-quality music at a 48kHz sampling rate. The integration of diffusion models and masked autoencoders further enhances JEN-1's ability to capture complex sequence dependencies in music. Our extensive quantitative and human evaluations demonstrate JEN-1's superiority over strong baselines in subjective quality, diversity, and controllability.
%The proposed prompt learning strategy enables accurate control over the generation process and facilitates precise text-to-music correspondence. % prompt embedding alignment? 创新点: input text -> 训练集text alignment; 类似于 codebook的码本? 创新点二: 多轨一致性 & cot, 通过提示工程把不同的任务、流派、标签这种外部信息迁移进去. 甚至可以借助语音数据值来辅助训练唱歌数据集.创新点三: 多轨里面额外加入人声轨,多种乐器和人声轨统一的大模型.
JEN-1 also excels at music completion and continuation tasks under the multi-task training regime. These results highlight the effectiveness of our techniques in modeling music waveforms and the advantages of the unified framework.

This research pushes the frontier of text-to-music generation and provides a compelling solution for high-quality, semantically controllable music synthesis from text. Potential future directions include incorporating external knowledge to enhance controllability and extending the framework to other cross-modal generation tasks. We hope our work will inspire more efforts in developing generative models that create impactful and realistic art. As text-to-music generation matures from research into practical applications, it bears great potential to augment human creativity and reshape how people compose, share, and appreciate music.

%%%%%%%%%%%%%%%%%%%%%%simple version%%%%%%%%%%%
% In this work, we propose JEN-1, a text-to-music framework that directly models waveforms and integrates autoregressive and non-autoregressive training. Through multi-task objectives, JEN-1 achieves high-quality music generation from text descriptions. Extensive evaluations show JEN-1's superiority in quality, diversity, and controllability over strong baselines. This research advances the state-of-the-art in controllable text-to-music generation.

% Future directions include exploring hierarchical music separation and external knowledge incorporation. We believe high-quality text-to-music generation will empower new creative workflows and reshape music composition and appreciation. As the field matures from research to practical applications, it bears great potential to augment human creativity.
